Effectively Searching Maps in Web Documents

Maps are an important source of information in archaeology and other sciences. Users want to search for historical maps to determine recorded history of the political geography of regions at different eras, to find out where exactly archaeological artifacts were discovered, etc. Currently, they have to use a generic search engine and add the term map along with other keywords to search for maps. This crude method will generate a significant number of false positives that the user will need to cull through to get the desired results. To reduce their manual effort, we propose an automatic map identification, indexing, and retrieval system that enables users to search and retrieve maps appearing in a large corpus of digital documents using simple keyword queries. We identify features that can help in distinguishing maps from other figures in digital documents and show how a Support-Vector-Machine-based classifier can be used to identify maps. We propose map-level-metadata e.g., captions, references to the maps in text, etc. and document-level metadata, e.g., title, abstract, citations, how recent the publication is, etc. and show how they can be automatically extracted and indexed. Our novel ranking algorithm weights different metadata fields differently and also uses the document-level metadata to help rank retrieved maps. Empirical evaluations show which features should be selected and which metadata fields should be weighted more. We also demonstrate improved retrieval results in comparison to adaptations of existing methods for map retrieval. Our map search engine has been deployed in an online map-search system that is part of the Blind-Review digital library system.

==> abs.tex <==
Maps are an important source of information in archaeology and
other sciences.  Users want to search for historical maps to
determine recorded history of the political geography of regions
at different eras, to find out where exactly archaeological artifacts
were discovered,  etc.  Currently, they have to use a generic search engine
and add the term map along with other keywords to search for maps.
This crude method will generate a significant number of false positives
that the user will need to cull through to get the desired results.
To reduce their manual effort, we propose an automatic map 
identification, indexing, and retrieval system that enables users to
search and retrieve maps appearing in a large corpus of
digital documents using simple keyword queries.
We identify features that can help in distinguishing maps from other
figures in digital documents and show how a Support-Vector-Machine-based
classifier can be used to identify maps.  We propose map-level-metadata
e.g., captions, references to the maps in text, etc. and document-level
metadata, e.g., title, abstract, citations, how recent the publication is, etc. and
show how they can be automatically extracted and indexed.  
Our novel ranking algorithm weights different metadata fields differently
and also uses the document-level metadata to help rank retrieved maps.
Empirical evaluations show which features should be selected and which 
metadata fields should be weighted more.  We also demonstrate improved
retrieval results in comparison to adaptations of existing methods for 
map retrieval.  Our map search engine has been deployed in an online
map-search system that is part of the Blind-Review digital library system.

==> sec2_rel.tex <==
\vv\section{Related Work}\label{sec2_rel} In this section, we will
discuss related work.

\textbf{Existing Related Systems}. Much work has been done in the field of
map data processing. A system used for acquisition, storage, indexing, and
retrieval of map images is described in~\cite{samet98ijdar}. The inputs to
their system are raster images of maps. These images are then stored as a
record containing map related information in a relational database.
Advanced database techniques from the field of spatial databases are
adopted to build indices. Queries are posed to the system using an
SQL-like language. In~\cite{lim02jcdl}, a G-Portal system is set up to
identify, classify, and organize geo-spatial and geo-referenced content on
the World Wide Web. A digital library can access these data by using a
map-based interface. A legend-driven map interpretation system, MARCO (MAp
Retrieval by COntent), is proposed in \cite{samet96itpami} to convert map
images from their physical representation to their logical representation.
The logical representation is then stored and used to build index. R. P.
Futrelle has set up a diagram understanding system to understand diagrams
in technical documents \cite{futrelle92computer,futrelle07tr}. This is the
first such system to fully parse a variety of actual diagrams drawn from
the research literature. Digmap
system\footnote{http://code.google.com/p/digmap/} \cite{gir07martins} is a
geographic IR system based on the historical digitized maps.

Our work is different from those we described above. In their approaches,
the information is dynamically extracted from either paper-based maps or
digital maps on the Web. They consider maps in isolation, i.e., excluding
other content in digital documents. In contrast, we extract maps from
digital documents and utilize the ``context'' of the maps like captions
and references in the text, as well as other context-based boosting
factors depending on the digital documents, to get hints on understanding
their contents. Our experiment results show that inclusion of these
factors can significantly improve the map retrieval performance. The
DIGMAP system takes into account some textual description of the maps.
However, these descriptions are provided along with the maps. DIGMAP does
not consider the problem of extracting maps and the related map metadata
from documents, as well as the problem of distinguishing maps from other
images in a document. Both of these problems are critical because a large
number of maps are embedded in documents.
%This leads to the limitation of DIGMAP application and methods.

There is another online map search online
system\footnote{http://scilsresx.rutgers.edu/~gelern/maps/}~\cite{jcdl08gelernter},
which was motivated in part by discussions with our team, in which maps
are also extracted from some Web documents in PDF format The maps are
indexed based on maps' content in three dimensions, region, time period,
and theme. However, this project is just starting and no details of the
design or implementation are discussed in~\cite{jcdl08gelernter}.

%\textbf{Image Retrieval}. Because most maps are shown in a digital
%document as an image, our work is related to image retrieval. Early
%approaches for image retrieval were text-based approaches. Usually, user
%annotations were manually added to pictures and search was performed using
%a standard database management system~\cite{chang80tse,roussopoulos88tse}.
%With the growth of image databases, however, manually annotating all
%images became impractical. Interest in image retrieval shifted toward
%content-based approaches~\cite{rui99jvcair,wang00visual}. Content-based
%image retrieval is based on extracting image features, such as color,
%texture, or shape, from the objects in the database. The extracted
%features are then stored and compared to a query image expressed using a
%feature description language~\cite{aslandogan99tkde}. The various
%proposals based on content-based retrieval differ mainly on the techniques
%used for extracting and storing
%features~\cite{ogle95computer,wu97tkde,kwae00tis} and on the use of such
%features for image
%search~\cite{flickner95computer,cox00tip,santini00multimedia,wang00visual}.
%Our work differs from this type of technique in that we define a set of
%metadata to index the maps, extract them automatically, and consider each
%type of metadata as an individual source of evidence, which we then
%combine and access through a novel ranking function.
%
%There are also existing works on map
%analysis~\cite{docprocs88bixler,survey00fortier,grec01cao,grec01aurelio,gis05chiang}.
%In these work, methods are proposed to separate and recognize the
%touching/overlapping alphanumeric characters from maps. These are
%important implementations in map analysis. However, they did not explain
%how to use the extracted characters to perform retrieval. Nor did they
%consider related text other than the extracted words.
%In future work, we will
%consider indexing text extracted from inside the map.

\textbf{Multimodal/Structured Document Retrieval}. Our work is also
related to indexing and retrieving images for multimodal digital
documents. Multimodal documents convey information using both text and
images. Different Information Retrieval (IR) techniques have been used to
build up, index and retrieval functions. Some of these existing works deal
with only the text in the document and ignore all the image-related
information~\cite{witten99mg}. Some of them deal with only images, as in
content-based image retrieval (CBIR)~\cite{smeulders00tpami}. Others use
both text and image objects~\cite{mitra00ir}.
%In our work, we limit
%our techniques to the text in the digital documents due to the constraint
%that there is no reliable tool so far to accurately extract content
%of images from a scanned PDF document. %Even there are some tools
%under developing, it could be too computationally expensive for a
%general map search system. Unlike image, text have been extracted
%from scanned PDF document by using OCR tools. Although there are
%still some inaccuracy in OCR, the results come out much more
%satisfying.
Current OCR tools were not very effective in extracting text from maps in
our preliminary experiments. In the future, we will extract and index text
lying inside maps. Once such information is extracted, our current
framework can index and utilize them seamlessly.

As discussed in Section~\ref{sec6_index}, we consider the map metadata as
various information fields for a map, and propose a structured document
retrieval technique to build a map index. Therefore, we now discuss
related work on structured document retrieval briefly. A document is said
to be structured when it contains multiple fields. A document's field
structure is commonly used to improve retrieval performance in practice.
%There are two kinds of existing work for this area. First,
The most commonly used approach for structured document retrieval is a
score/rank linear
combination~\cite{wilkinson94sigir,myaeng98sigir,lalmas00tr,wu07ipm},
which treats each field as a separate document and computes a combined
scores/ranks.
%%% check the sentence above to make sure it's what is meant
In computing scores for each field, any ranking function for unstructured
document retrieval can be adopted. Another approach is to essentially
combine term frequencies instead of scores. In~\cite{robertson04cikm}, an
extension of the BM25 formula is introduced and is a simple and efficient
method which combines term frequencies instead of field scores.
In~\cite{ogilvie03sigir}, within the language model framework, this
approach proposes a separate language model for each field and then
combines them linearly. Our work adopts and extends these two pieces of
work and proposes novel retrieval functions for the map search system.


==> sec4_meta.tex <==
\vv\vv\vv\vv\vv\vv\section{Automatic Metadata Extraction}\label{sec4_meta} The text
associated with an image in a document can help interpret the image
better. We define two sets of metadata: map level metadata generated
from the text accompanying the map, and the host document level metadata.
\vv\vv\subsection{Map Level Metadata} We consider the following map-level
metadata: the caption, the reference text, and the document page
containing the map. These three entities can be used for identifying as
well as retrieving maps. They are listed as follows, ordered by the
likelihood of being useful during a map search. \vv\begin{itemize}
\item \textit{Map caption}.
\item \textit{Map reference}. We use the term {\it map reference}
to refer to text in the document that refers to the map. We denote a
phrase like ``Figure 1'' or ``Fig 1'' in the main body as the
\textit{reference point}, and we define the map reference text as the
sentence which contains this reference point. %If the unit equals
%to 2, the reference text is the two sentences which are the most
%closed to the reference point.
%We note that all the reference text should be in the same paragraph.
\item \textit{Map size}.
We use a relative instead of absolute percentage value to represent the
map size. Suppose the number of text lines in a page without any figure is
$N_T^{nf}$, and the number of text lines in a page with $N_F^f$ figures is
$N_T^f$, then the average size of each figure can be computed as
$\frac{1-N_T^f/N_T^{nf}}{N_F^f}$.
\item \textit{Map figure number and document page number}.
\end{itemize}\vv

%To extract map level metadata, the major task is to extract the map's
%caption and the reference text. In our work, we define the following
%heuristic rules for these two types of extractions.

First, to extract the caption of a map, we consider each line as a unit
and try to identify whether a unit belongs to the classes
``caption\_begin", ``caption\_end", or ``other". A unit is tagged as
caption\_begin if all of the following conditions are satisfied: 1) it
begins with ``Figure'', ``FIGURE'', ``Fig'', or ``FIG'' + a number; 2) its
font and fontsize are both different from those of the previous unit; and
3) its font size is smaller than that of the document's regular size.
Alternatively, a unit is tagged as caption\_end if all of the following
conditions are satisfied: 1) it ends with ``.''; 2) its font and fontsize
are both different from those of the following unit; 3) its font size is
smaller than that of the document's regular size; and 4) all units between
the current unit and the most previous caption\_begin unit are in the same
paragraph and have the same presentation, i.e., the same font and font
size. Lines lying between the unit caption\_begin to the unit labeled
caption\_end comprise the caption of a figure.
%\begin{itemize}
%
%\item \textit{Font Size change}: The size of previous line is different to the current one if the
%current one is the beginning of the caption. The size of the following line is different
%to the current one if the current one is the end of the caption. Combining this rule with the first
%one, we can easily extract the while body of the caption. ;
%\item \textit{Boldface}: Captions are written in boldface;
%\item \textit{Alignment}: The current line has centered alignment;
%\item \textit{Alignment Change}: The lines either preceeding the caption or following
%the caption has left alignment;
%\item \textit{Same Paragraph}: Lines in a caption locates in the same paragraph. To
%get the paragraph, we can make use of the alignment information.
%\end{itemize}

We define another set of heuristic rules for the reference text
extraction. Given a map's figure number and its host document, we first
figure out the reference point in the document body by using the following
rules: 1) \textit{Key Words}: The reference point is tagged with
``Figure'', ``FIGURE'', ``Fig'', or ``FIG'' and followed by the figure
number of the map; and 2) \textit{Font Size}: The font size of the
reference is the same as the regular size of the document. Based on the
second rule, we avoid mistaking the map's caption for the map's reference.
%\item \textit{Alignment}: The current line has left alignment;
%3) \textit{Same Paragraph}: Lines in a map's reference text locates in the same paragraph.
Once we have acquired the reference point, we extract the sentence
containing the reference point as the map's reference text.

\vv\vv\subsection{Document Level Metadata} Our system extracts document
level metadata comprising of the \textit{title}, \textit{abstract},
\textit{author}, \textit{ publication date}, and \textit{citations}. In
response to users' search queries, the document-level metadata is used to
assist in the search (see Section~\ref{sec6_index}). We built learning
models to extract document level metadata, as those used in existing
digital libraries~\cite{councill06jcdl}. The extraction process is not the
focus of our paper.


==> sec5_identify.tex <==
\vv\section{Map Identification}\label{sec5_identify} In this section, we
outline an algorithm to identify maps from among other figures using a
two-class classifier
%Support Vector Machine (SVM) classifier~\cite{joachims99book}
on a set of features. %, which are extracted from the map metadata.

\vv\subsection{Features Extraction} We consider two categories of
features for the classifier: basic term-based features and advanced
features. First, the algorithm removes stop words, stems words, and
eliminates from the vocabulary the terms that appear only once in the
whole set of documents. Preprocessing reduces the dimension of the feature
vectors by removing terms not helpful in identifying a map.

\textbf{Basic Features}. The algorithm uses a set of basic features
corresponding to the frequencies of the terms in the text. A \textit{term}
is defined to be any alphabetical sequence of characters separated by
non-alphabetical characters such as white space. Terms are generated by
splitting the text at any non-alphabetical character. The algorithm uses
three categories of basic term features extracted from (i) captions, (ii)
references, and (iii) a combination of both.

\textbf{Advanced Features}. We use the following advanced features:
\vv\begin{itemize}
\item \textit{BeginsWith}. This feature is 1 for the first term in
a caption and 0 for rest of the terms.
\item \textit{FigureNO}. This is one binary
feature indicating whether or not the figure's number falls within the
range [1,2].  This feature is specific to the archaeology domain. We have
observed that usually the first figure of an archeology paper is a map
because the paper tends to introduce the geographical information, and
then present other related information.
\item \textit{LocationNames}. These are two sets of
binary features calculating how many words related to locations are used
in the figure's caption and reference, respectively. Typically, the text
explaining the figure will contain more location-related words if the
figure is a map. We use GATE\footnote{http://gate.ac.uk/} to tag location
names in the caption/reference. Next, the number of tagged location names
are separated to six intervals: [0], [1,2], [3,5], [5,9], [10, 20],
$\-[21, \infty]$. We define one binary feature for each interval. For
instance, if the number of tagged location names falls within a specific
interval, the corresponding feature becomes 1 while all other five
features remain 0.
\item \textit{Size}. This is a binary feature indicating whether or not
the image size is larger than $1/3$ of the entire page. We have observed
that most large figures in archeology papers are maps because maps bear
geographical details, which are usually more complex than figures and
require more space for illustrations.
\end{itemize}\vv

\vv\subsection{SVM Classification}
The number of features could be too large for training the model
efficiently and labeling other figures. To address this issue, we adopt a
statistical method, namely expected entropy loss~\cite{abramsn63itc}, to
select only the features that are effective for the training process.

Expected entropy loss is computed separately for each feature. %Let $C$
%be the event that indicates whether a figure is a member of the
%map class and let $f$ be the event that the
%figure contains the specified feature. Let $\overline{C}$ and
%$\overline{f}$ be their negations. We can compute their probability as,
%\begin{eqnarray}\label{equ_pro}
%Pr(C)&=&\frac{\#~of~Positive~Samples}{\#~of~Samples}  \nonumber\\
%Pr(\overline{C})&=&1-Pr(C) \nonumber\\
%Pr(f)&=&\frac{\#~of~Samples~With~Feature~F}{\#~of~Samples}  \nonumber\\
%Pr(\overline{f})&=&1-Pr(f) \nonumber\\
%Pr(C|f)&=&\frac{\#~of~Positive~Samples~With~Feature~F}{\#~of~Samples~With~Feature~F}  \nonumber\\
%Pr(\overline{C}|f)&=&1-Pr(C|f) \nonumber\\
%Pr(C|\overline{f})&=&\frac{\#~of~Positive~Samples~Without~Feature~F}{\#~of~Samples}  \nonumber\\
%Pr(\overline{C}|\overline{f})&=&1-Pr(C|\overline{f}) \nonumber\\\nonumber
%\end{eqnarray}
%The prior entropy of the class distribution is
%\begin{equation}\label{equ:prior}
%    e = -Pr(C)\lg(Pr(C))-Pr(\overline{C})\lg(Pr(\overline{C})) \nonumber
%\end{equation}
%The posterior entropy of the class when feature is present is
%\begin{equation}\label{equ:post}
%    e_f = -Pr(C|f)\lg(Pr(C|f))-Pr(\overline{C}|f)\lg(Pr(\overline{C}|f)) \nonumber
%\end{equation}
%likewise, the posterior entropy of the class when the feature is
%absent is
%\begin{equation}\label{equ:post}
%    e_{\overline{f}} =
%    -Pr(C|\overline{f})\lg(Pr(C|\overline{f}))-Pr(\overline{C}|\overline{f})\lg(Pr(\overline{C}|\overline{f})) \nonumber
%\end{equation}
%Thus the expected posterior entropy is
%\begin{equation}\label{equ:post}
%    e_fPr(f)+e_{\overline{f}}Pr(\overline{f}) \nonumber
%\end{equation}
%and the expected entropy loss is
%\begin{equation}\label{equ:post}
%    e-e_fPr(f)+e_{\overline{f}}Pr(\overline{f}) \nonumber
%\end{equation}
%
Then, we rank the features according to their expected entropy loss.
Features that are common in both the positive set and the negative set
rank lower, while they rank higher if they are effective in discriminating
the positive class from the negative one. This approach has been generally
adopted for feature selection before training a
classifier~\cite{krovetz03sigir}. We compute the expected entropy loss for
each feature and sort all the features by expected entropy loss in
descending order. Through setting a threshold, we get feature sets of
different sizes. In our experiment, we will test the effectiveness of
tuning the size of the feature set.

We consider the map identification process as a classification process
that categorizes images into two groups, maps and non-maps. Our system
identifies maps using a supervised classifier. First, we train a
classifier on the feature vectors generated from the training set in which
each image has a class label indicating whether it is a map or not. This
classifier is then used to test other images. Cross
validation~\cite{devijver82book} is used for the training and the testing
process.

We use Support Vector Machines(SVMs), which are learning machines used for
two-group classification problems~\cite{ml95cortes}. SVMs have been
proved to be the most applicable tool for text categorization problems
because they can handle high dimensional feature vectors, reduce problem
caused by over-fitting, and produce solutions that are robust to
noise~\cite{joachims99book}. For our problem, we assume that the
classification problem is linearly separable. That is, the set of training
data in a high-dimensional space can be classified into two classes by a
separating hyperplane. Therefore, to solve the classification problem, it
is necessary to construct such an optimal hyperplane in a high-dimensional
space.


==> sec8_conc.tex <==
\vv\vv\section{Conclusions and Future Work}\label{sec8_conc}

We have proposed a novel system that enables searching for maps in digital
academic documents. We select a set of features that help identify maps.
Our system first extracts figures from documents and classifies them as
maps and non-maps. It identifies the caption and references of the maps
and indexes them.  We have proposed a ranking function that utilizes the
captions and references of the maps, as well as document-level features
like the document title, document age, document popularity and importance
of publication venues to enable map search. Experimental results performed
on JSTOR archaeology journal document show the effectiveness of our chosen
features and ranking methods.

In the future, there are several interesting directions to pursue. First,
we plan to include image analysis tools for indexing and utilizing text
appearing inside the maps themselves. Second, we realize that different
classification algorithms may have different impacts on map
identification. We will investigate other classifiers besides SVM and find
the most suitable for our application. Finally, we will look into location
keywords and take into account spatial queries in the map retrieval
system.

